PASTA: A Parallel Sparse Tensor Algorithm Benchmark Suite

Tensor methods have gained increasingly attention from various applications, including machine learning, quantum chemistry, healthcare analytics, social network analysis, data mining, and signal processing, to name a few. Sparse tensors and their algorithms become critical to further improve the performance of these methods and enhance the interpretability of their output. This work presents a sparse tensor algorithm benchmark suite (PASTA) for single- and multi-core CPUs. To the best of our knowledge, this is the first benchmark suite for sparse tensor world. PASTA targets on: 1) helping application users to evaluate different computer systems using its representative computational workloads; 2) providing insights to better utilize existed computer architecture and systems and inspiration for the future design. This benchmark suite is publicly released https://gitlab.com/tensorworld/pasta.

==> src/tab-libs.tex <==
\begin{table} % <-- HERE
\centering
\footnotesize
    \begin{tabular}{ |l  c  c  c  c  c  c  l  c  l|}
    \toprule 
    % \hline
    \multirow{2}{*}{\textbf{Software}} & \multicolumn{5}{c}{\textbf{Workloads}} & \multirow{2}{*}{\textbf{Order}} & \multirow{2}{*}{\textbf{Parallelized}} & \multicolumn{2}{c}{\textbf{Software Info.}} \\ \cline{2-6} \cline{9-10}

    & \TEW & \TS & \TTV & \TTM & \MTTKRP & & & \textbf{Domain} & \textbf{Environ.} \\
    \midrule
    Numpy~\cite{numpy,numpy-paper,numpy-web}             
    & \yesy & ? & ? & \non & \non & Arb. & \non & Gen. & Python \\ \myhline
    scikit-tensor~\cite{scikit-tensor-web}             
    & \yesy & ? & ? & \yesy & \non & Arb. & \non & Gen. & Python \\ \myhline
    PyTensor~\cite{Yoo10pytensor:a,doi:10.1021/ct100531j,PyTensor}             
    & \non & ? & ? & \yesy & \non & Arb. & \non & Sim. & Python \\ \myhline
    TCE (NWChem)~\cite{TCE,TCE-web}
    & \yesy & ? & ? & \yesy & \non & $\leq 4$ & \yesy ~$^{2,3}$ & Chem. & DSL \\ \myhline
    libtensor~\cite{libtensor-paper1,libtensor}      
    & \yesy & ? & ? & \yesy & \non & Arb. & \yesy ~$^1$ & Gen. & C/C++ \\ \myhline
    CTF~\cite{solomonik2014massively,CTF-web}
    & \yesy & ? & ? & \yesy & \non & Arb. & \yesy ~$^{1,2,3}$ & Gen. & C/C++ \\ \myhline
    TiledArray~\cite{Calvin:2015,tiledarray}
    & \yesy & ? & ? & \yesy & \non & Arb. & \yesy ~$^{1,2}$ & Gen. & C/C++ \\ \myhline
    TL (Dynare++)~\cite{dynpp_tl,tl_Dynare-web}
    & \yesy & ? & ? & \yesy & \non & Arb. & \yesy ~$^{1}$ & FIN & C/C++ \\ \myhline
    SPLATT~\cite{smith2016splatt,SPLATT-web}
    & \non & ? & ? & \non & \yesy & Arb. & \yesy ~$^{1,2}$ & Gen. & C/C++ \\ \myhline
    DFacTo~\cite{NIPS2014_5395,DFacTo-web}
    & \non & ? & ? & \non & \yesy & $\leq 3$ & \yesy ~$^{1}$ & Gen. & C/C++ \\ \myhline
    HaTen2~\cite{haten2_ICDE2015,HaTen2-web}
    & \non & ? & ? & \yesy & \yesy & $\leq 3$ & \yesy ~$^{2}$ & ML & JAVA \\ \myhline

    Tensor Toolbox~\cite{TTB_Dense,Bader07efficientmatlab,TTB_Software}
    & \yesy & ? & ? & \yesy & \yesy & Arb. & \non & Gen. & MATLAB \\ \myhline
    PLS\_Toolbox~\cite{PLS-toolbox}
    & \yesy & ? & ? & \yesy & \non & Arb. & \non & Chem. & MATLAB \\ \myhline
    TT-Toolbox~\cite{tt-toolbox}
    & \yesy & ? & ? & \yesy & \non & Arb. & \non & Gen. & MATLAB \\ \myhline
    H-Tucker~\cite{Kressner:2014:A9H:2610268.2538688,HT} 
    & \yesy & ? & ? & \yesy & \non & Arb. & \non & Gen. & MATLAB \\ \myhline
    Tensorlab~\cite{Tensorlab}
    & \yesy & ? & ? & \yesy & \yesy & Arb. & \yesy ~$^{1}$ & Gen. & MATLAB \\ \myhline
    TDALAB~\cite{TDALAB,TDALAB-web}
    & \yesy & ? & ? & \non & \non & Arb. & \non & Gen. & MATLAB \\ \myhline
    TENSORBOX~\cite{TENSORBOX}
    & \yesy & ? & ? & \yesy & \yesy & Arb. & \non & Gen. & MATLAB \\ \myhline
    ITensor~\cite{itensor}
    & \yesy & ? & ? & \yesy & \non & Arb. & \non & Sim. & C/C++ \\ \myhline
    TensorLy~\cite{xx}
    & ? & ? & ? & ? & ? & Arb. & ? & ? & ? \\
    \bottomrule
    \end{tabular}
\caption*{ \footnotesize{
\textbf{MTTKRP}: Optimized MTTKRP kernel;~~~~~~~~ \textbf{Order}: Arb. - Arbitrary;~~~~~~~~ \textbf{Environ.}: DSL - Domain Specific Language;\\
\textbf{Sparse}: $^*$Block-wise Sparsity; Otherwise, Element-wise Sparsity; \\
\textbf{Parallelized}: $^1$Multi-Threading Parallelism;~~~~~~~~ $^2$Distributed Parallelism;~~~~~~~~ $^3$Accelerator Parallelism\\
\textbf{Domain}: Gen. - General;~~~~ Sim. - Simulation;~~~~ Chem. - Chemistry;~~~~ ML - Machine Learning;~~~~ FIN - Finance;
}}
\caption{Capabilities of tensor frameworks as of submission date.}
\label{tab:libs}
\end{table}
%\footnotetext[1]{Multi-threading Parallelism}
%\footnotetext[2]{Distributed Parallelism}
%\footnotetext[3]{Accelerator Parallelism}
